Planted: a dataset for planted forest identification from multi-satellite time series

Protecting and restoring forest ecosystems is critical for biodiversity conservation and carbon sequestration. Forest monitoring on a global scale is essential for prioritizing and assessing conservation efforts. Satellite-based remote sensing is the only viable solution for providing global coverage, but to date, large-scale forest monitoring is limited to single modalities and single time points. In this paper, we present a dataset consisting of data from five public satellites for recognizing forest plantations and planted tree species across the globe. Each satellite modality consists of a multi-year time series. The dataset, named \PlantD, includes over 2M examples of 64 tree label classes (46 genera and 40 species), distributed among 41 countries. This dataset is released to foster research in forest monitoring using multimodal, multi-scale, multi-temporal data sources. Additionally, we present initial baseline results and evaluate modality fusion and data augmentation approaches for this dataset.

==> datasheet_reduced.tex <==

\section{Datasheet for dataset \PlantD}
\label{app:dataset-docu}

This dataset datasheet is based on the recommended methodology from Gebru et al \cite{gebru2021:datasheets}. The prompts from \cite{gebru2021:datasheets} are in \dsq{blue} and our answers are in black.

\subsection{Motivation}
\dsq{\textbf{For what purpose was the dataset created?}
Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.}

\PlantD\ was created to foster AI research in remote sensing of forests, using multimodal, multi-scale, multi-temporal data sources. In order to advance global forest understanding to support biodiversity conservation and carbon sequestration challenges.


\dsq{\textbf{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}}

The dataset was created by a research team in Google DeepMind with support from volunteer contributors in Google Research and Mineral AI.





\subsection{Composition}

\dsq{\textbf{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}
Are there multiple types of instances (e.g., movies, users, and ratings; people and interactions between them; nodes and edges)? Please provide a description.}

The instances represent forest patches of planted forests and tree crops around the world, with an extent of 120m x 120m.

Each example consists of multimodal time series from 5 satellites (Sentinel-1, Sentinel-2, Landsat-7, ALOS-2 PALSAR-2, MODIS Terra/Aqua), including forest plantation and tree crops labels (species name, common name, tree traits) and auxiliary data (location, times of satellite data acquisition, validity masks for satellite data).

\dsq{\textbf{How many instances are there in total (of each type, if appropriate)?}}

There are 2,264,747 instances in total.

\dsq{\textbf{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}
If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g., geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g., to cover a more diverse range of instances, because instances were withheld or unavailable).}

This dataset is based on a filtered subset of the Spatial Dataset of Planted Trees (SDPT)~\cite{Harris:sdpt}, where we discarded all samples that have been generated by another ML model. Other filtering criteria include knowing exactly the single monoculture species, the forest plantation had to be at least 1/4 hectares, there should be at least 10 samples per species type. The examples locations have additionally been de-duplicated, keeping only a single sample within a small local cluster.

\dsq{\textbf{What data does each instance consist of?}
“Raw” data (e.g., unprocessed text or images) or features? In either case, please provide a description.}

Each example consists of multimodal time series from 5 satellites (Sentinel-1, Sentinel-2, Landsat-7, ALOS-2 PALSAR-2, MODIS Terra/Aqua), including forest plantation and tree crops labels (species name, common name, tree traits) and auxiliary data (location, times of satellite data acquisition, validity masks for satellite data). Exact details on the dimensions, types, and descriptions can be found in the main paper in Section 3.1 and in Table 1.


\dsq{\textbf{Is there a label or target associated with each instance?}
If so, please provide a description.}

Yes, each example is annotated with the monoculture species name, common name, as well as an indication whether it is coniferous, broadleaf, evergreen, decidious, hard or soft wood. If some of the secondary information is not known, then the \textit{Unknown} label is found.

\dsq{\textbf{Is any information missing from individual instances?}
If so, please provide a description, explaining why this information is missing (e.g., because it was unavailable). This does not include intentionally removed information, but might include, e.g., redacted text.}

Some satellite data is missing, due to various reasons (strong cloud coverage, limited satellite coverage) --- it is discussed in more detail in \autoref{app:missing-data}. Some secondary labels are missing - they are not considered critical and were not provided in the upstream data.

\dsq{\textbf{Are relationships between individual instances made explicit (e.g., users’ movie ratings, social network links)?}
If so, please describe how these relationships are made explicit.}

The spatial and temporal information for each satellite data source is provided via latitude, longitude and time series timestamps and dates of data acquisition.

\dsq{\textbf{Are there recommended data splits (e.g., training, development/validation, testing)?}
If so, please provide a description of these splits, explaining the rationale behind them.}

Yes, the examples were distributed into three splits (train, validation, and test), with a reference ratio of 8:1:1, respectively. However, to ensure reliable evaluation, for low samples regime (<100 total examples), we used 1:1:1 ratio, and we limit the number of validation and test examples to about 1000. We used an adaptive geographic splitting approach, first dividing the world into regions of approximately 20x20 km (400 km${}^2$) to 80x80 km (6400 km${}^2$) (depending on how many such regions we got per label), and assigning all samples within one such region randomly to one of the three splits. The distribution of labels across the splits is available in \autoref{app:details-labels}.

\dsq{\textbf{Are there any errors, sources of noise, or redundancies in the dataset?}
If so, please provide a description.}

Satellite data has to be considered noisy, and it is part of the challenge to be able to develop robust approaches that can handle that noise. Label data might be inaccurate, and the exact time of data labeling is unknown (within 2013-2015), so that it's possible that the satellite data shows modified land use state if there was change between data labeling and satellite data acquisition.

\dsq{\textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?}
If it links to or relies on external resources, a) are there guarantees that they will exist, and remain constant, over time; b) are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created); c) are there any restrictions (e.g., licenses, fees) associated with any of the external resources that might apply to a future user? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.}

The dataset is self contained.

\dsq{\textbf{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals’ non-public communications)?}
If so, please provide a description.}

To the best of our knowledge, this dataset does not contain confidential information. All data sources are already in the public domain.

\dsq{\textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}
If so, please describe why.}

No.

\dsq{\textbf{Does the dataset relate to people?}
If not, you may skip the remaining questions in this section.}

No.









\subsection{Collection process}

\dsq{\textbf{How was the data associated with each instance acquired?}
Was the data directly observable (e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or language)? If data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.}

The forest plantation and tree crop species types have already been collected and harmonized in the \textit{Spatial Database of Planted Trees} \cite{Harris:sdpt} and is publicly available. 
























\subsection{Preprocessing/cleaning/labeling}

\dsq{\textbf{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?}
If so, please provide a description. If not, you may skip the remainder of the questions in this section.}

The preprocessing of satellite data is outlines in Section 4.1. It included for Sentinel-2 and Landsat-7 construction of cloud-free mosaics for each season time range (3 months). Sentinel-1 and MODIS data was time-averaged over the given time ranges (seasonal for Sentinel-1 and monthly for MODIS). Each satellite data was projected on local UTM coordinates, resampled to satellite-dependent resolution, and the imagery of a 120m x 120m square was extracted around the centroid of forest plantation. For each satellite, a mask distinguishing valid pixels from invalid was created. For each satellite image time sample, the average time (timestamp and date) of the date range (monthly, seasonal, or yearly) was extracted and added to all instances. We kept all satellite data units and value ranges the same as provided by Google Earth Engine.





















\subsection{Distribution}

\dsq{\textbf{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?}
If so, please provide a description.}

Yes, this dataset will be publicly available on the internet.

\dsq{\textbf{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)?}
Does the dataset have a digital object identifier (DOI)?}

The dataset will be made available via TFDS or github (TBD) and be downloadable from Google Cloud.
We do not yet have a DOI.



\dsq{\textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}
If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.}

The dataset will be distributed under the CC-BY-4.0 license.

\dsq{\textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}
If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.}

No, not to the best of our knowledge. 
The licences and terms of conditions for all used source data is below:
\begin{itemize}
\item SDPT labels data \cite{Harris:sdpt} license: CC-BY-4.0.
\item Landsat-7: Landsat datasets are federally created data and therefore reside in the public domain and may be used, transferred, or reproduced without copyright restriction.
Acknowledgement or credit of the USGS as data source should be provided by including a line of text citation such as the example shown below (\url{https://developers.google.com/earth-engine/datasets/catalog/LANDSAT_LE07_C02_T1_L2}). Acknowledgement:
"Landsat-7 image courtesy of the U.S. Geological Survey."
\item Sentinel-1: EU law grants free access to Copernicus Sentinel Data and Service Information for the purpose of the following use in so far as it is lawful: (a) reproduction; (b) distribution; (c) communication to the public; (d) adaptation, modification and combination with other data and information;(e) any combination of points (a) to (d) \url{https://scihub.copernicus.eu/twiki/pub/SciHubWebPortal/TermsConditions/Sentinel_Data_Terms_and_Conditions.pdf}. Acknowledgement: "Contains modified Copernicus Sentinel data 2015-2017 for Sentinel data."
\item Sentinel-2: EU law grants free access to Copernicus Sentinel Data and Service Information for the purpose of the following use in so far as it is lawful: (a) reproduction; (b) distribution; (c) communication to the public; (d) adaptation, modification and combination with other data and information;(e) any combination of points (a) to (d) \url{https://scihub.copernicus.eu/twiki/pub/SciHubWebPortal/TermsConditions/Sentinel_Data_Terms_and_Conditions.pdf}. Acknowledgement: "Contains modified Copernicus Sentinel data 2015-2017 for Sentinel data."
\item ALOS: JAXA retains ownership of the dataset and cannot guarantee any problem caused by or possibly caused by using the datasets. Anyone wishing to publish any results using the datasets should clearly acknowledge the ownership of the data in the publication (\url{https://developers.google.com/earth-engine/datasets/catalog/JAXA_ALOS_PALSAR_YEARLY_SAR#terms-of-use}). Acknowledgement: "ALOS PALSAR data courtesy of JAXA (Japan Aerospace Exploration Agency."
\item MODIS: MODIS data and products acquired through the LP DAAC have no restrictions on subsequent use, sale, or redistribution (\url{https://developers.google.com/earth-engine/datasets/catalog/MODIS_061_MOD09A1}, LP DAAC: {https://lpdaac.usgs.gov/products/mod09a1v061/}) \cite{modis}.
\end{itemize}




























==> figs/1_individual_perf.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/1_individual_perf.png}
    \caption{Individual satellite performance with augmentations (flip + temporal masking) and without any augmentations. \maxim{which augmentations?}.\todo{Restrict ylim eg. to 60-95\%?}}
    \label{fig:data-augment}
\end{figure}


==> figs/4_max_acc_by_num_satellites.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/4_max_acc_by_num_satellites.png}
    \caption{Accuracy of the best performing satellite combination in dependence of number of modalities.
    }
    \label{fig:max_acc_by_num_sats
\end{figure}



==> figs/6_gflops_by_fusion_type.tex <==

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figs/6_gflops_by_fusion_type.png}
    \caption{Measured number of flops vs the number of satellites used, both for Vanilla ViViT models and MBT models. The need for MBT models becomes critical as the number of modalities increases.}
    \label{fig:gflops_by_fusion_type}
\end{figure}


==> figs/SI_bs_lr.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/SI_bs_lr.png}
    \caption{Effect of batch size and learning rate on mean validation accuracy for individual satellites. We did not evaluate on groups of satellites.}
    \label{fig:SI_bs_lr}
\end{figure}

